Deep learning applied to computational mechanics: A comprehensive review, state of the art, and the classics

Three recent breakthroughs due to AI in arts and science serve as motivation: An award winning digital image, protein folding, fast matrix multiplication. Many recent developments in artificial neural networks, particularly deep learning (DL), applied and relevant to computational mechanics (solid, fluids, finite-element technology) are reviewed in detail. Both hybrid and pure machine learning (ML) methods are discussed. Hybrid methods combine traditional PDE discretizations with ML methods either (1) to help model complex nonlinear constitutive relations, (2) to nonlinearly reduce the model order for efficient simulation (turbulence), or (3) to accelerate the simulation by predicting certain components in the traditional integration methods. Here, methods (1) and (2) relied on Long-Short-Term Memory (LSTM) architecture, with method (3) relying on convolutional neural networks. Pure ML methods to solve (nonlinear) PDEs are represented by Physics-Informed Neural network (PINN) methods, which could be combined with attention mechanism to address discontinuous solutions. Both LSTM and attention architectures, together with modern and generalized classic optimizers to include stochasticity for DL networks, are extensively reviewed. Kernel machines, including Gaussian processes, are provided to sufficient depth for more advanced works such as shallow networks with infinite width. Not only addressing experts, readers are assumed familiar with computational mechanics, but not with DL, whose concepts and applications are built up from the basics, aiming at bringing first-time learners quickly to the forefront of research. History and limitations of AI are recounted and discussed, with particular attention at pointing out misstatements or misconceptions of the classics, even in well-known references. Positioning and pointing control of a large-deformable beam is given as an example.

==> 0-NOTES.tex <==
%\vspace{1cm}
\newpage
{\color{red}

\section{NOTES}
%{\bf NOTES}
\label{sc:NOTES}

Jump to \hyperref[para:abstract]{Abstract}

% \today
\href{https://drive.google.com/file/d/1oVX6GxmQonaDKVr1rBly-SIs_d9CEkW_/view}{Goodfellow 2016 Deep learning - notes.pdf}

\begin{itemize}
  
  \item \today : document access / compilation date
  
  \item
  2020.06.18:
  This figure appeared in both Section~\ref{sc:Oishi-summary} and in Section~\ref{sc:Oishi-method-2-application}; the second figure from Section~\ref{sc:Oishi-method-2-application} was moved here, with its caption incorporated into the text in Section~\ref{sc:Oishi-method-2-application}. 
  \begin{figure}[h!]
  	\centering
  	\includegraphics[]{./figures/Oishi-2017-weight-correction-error-reduction}
  	\caption{
  		\emph{Method 2, application phase} (Section~\ref{sc:Oishi-method-2-application})
  		%{\it Improved quadrature accuracy by weight-correction.} 
  		Distribution of error reduction ratio $R_{\rm error}$ Eq.\eqref{eq:Oishi-error-reduction-ratio} for the \sout{test} training set (patterns) (a) and the validation set (test patterns) (b). 
  		Red bars (``Optimized'') refer to the optimal weights used as targets for training.
  		Blue bars (``Estimated by Neuro'') refer to predicted weights by the trained neural network. 
  		$R_{\rm error} < 1$ indicate improved quadrature accuracy, which occurred for \SI{99}{\percent} of the elements in the training set, and for \SI{97}{\percent} of the elements in the validation set.
  		Very few elements had their accuracy worsened ($R_{\rm error} > 1$) when using the predicted quadrature weights. As only elements that admitted improved quadrature accuracy by optimal quadrature weight correction were included in the training set and validation set, there were no red bars (optimal weights) for $R_{\rm error} > 1$.  See also Fig.\ref{fig:Oishi-error}. \cite{Oishi.2017:rd9648}
  		{\footnotesize (Figure reproduced with permission of the authors.)}
  	}
  	\label{fig:Oishi-2017-weight-correction-results}
  \end{figure}
  
  \item
  {\color{red} 2019.12.06.  to complete.  {\bf keywords to use in abstract:} state of the art, transformer and attention structures for recurrent neural networks beyond LSTM, with clear parallelism between continuous and discrete RNNs, stochastic optimization, adaptive learning rate algorithms, gradient and quasi-Newton methods with stochastic line search.  we included the latest papers available within the time constraint for this review paper.
  	
  	neuroscientific modeling neuron activities, experimental root of ReLU, connection between linear combination of inputs and linear part of Volterra series.  misconceptions on Rosenblatt's contribution, the original Perceptron as a multi-neuron network, and its hardware implementation in the Mark I computer.  
  	
  	convenience for readers with exact page numbers in thick books and links to online papers, including open online reviews where available.
  	
  	a classic never dies: 
  	\begin{itemize}
  		\item 
  		Artificial neural network by \cite{Rosenblatt.1957}, \cite{Rosenblatt.1958}, \cite{Rosenblatt.1960}, \cite{Block1962a}, \cite{Block1962b}, \cite{Rosenblatt.1962}
  		
  		\item 
  		ReLu in neuroscience, from experiments by \cite{Furshpan1957}, \cite{Furshpan1959a}, \cite{Furshpan1959b} to models in \cite{Dayan.2001}
  		
  		\item 
  		SDG by \cite{Robbins1951b}
  		
  		\item 
  		SDG with momentum (``small heavy sphere'') by \cite{Polyak.1964} 
  		
  		\item 
  		Goldstein, Armijo and Wolfe line search methods: \cite{Goldstein.1965}, \cite{Armijo.1966}, \cite{Wolfe.1969}
  	\end{itemize}
  	
  }
  
  \item
  2020.03.06. moved this figure back to NOTES.  i agreed that it did not add anything to the understanding of \cite{Oishi.2017:rd9648}.
  
  2019.12.10
  Mark: 01-motivation.tex, illustration of randomly distorted elements
  \begin{figure}[H]
  	\centering
  	\includegraphics[width=0.6\textwidth]{figures/training-set-hexa-individual-distorted.png}
  	\caption{
  		Training set formed by \num{5000} individual, randomly distorted and oriented hexahedral elements that are not connected into a finite element mesh. Figure created based on the two subfigures in Fig.\ref{fig:Oishi-hexahedral} just as an illustration.  Most people would think of elements in Fig.\ref{fig:Oishi-hexahedral} as part of a connected finite-element mesh, which is not the case.
  		\\
  		{\color{blue} [NOTE: 2019.06.10:
  			I'm not sure if the figure is necessary for for the understanding of Oishi's paper. In fact, it may be misunderstood since only two element shapes are illustrated. ENDNOTE]
  		}
  		\\
  		{\color{red} 2020.02.17.  
  			That was how i understood Fig.\ref{fig:Oishi-error}, since Fig.\ref{fig:Oishi-hexahedral} is confusing.  Remember, we are writing for first-time learners / readers, not for someone who already read the paper 10 times.  Without this figure, it is not clear how to get the statistics in Fig.\ref{fig:Oishi-error}.  We can discuss.
  		}
  	}
  	\label{fig:training-set-hexa}
  \end{figure}
  
  \item
  2020.01.13. moved the items with different fonts outside of the file 0-NOTES.tex and into the file fonts-test.tex, called by the master file fonts-many.tex.  cleaned up the file main.tex regarding math packages to get the command \verb|\mathfrak| working.
  
  \item 
  The following description of early stopping summarizes the above discussion:
  \begin{quote}
  	``Take an independent validation set, e.g. take out a part of the training set, and monitor the error on this set during training. The error on the training set will decrease, whereas the error on the validation set will first decrease and then increase. The early stopping point occurs where the error on the validation set is the lowest. It is here that the network weights provide the best generalization.''  \vphantom{\cite{Montavon.2012}}\cite{Montavon.2012}, p.49. 
  	%Preface to chapter on ``Regularization Techniques to Improve Generalization''.
  \end{quote}
  
  
  \item 
  2019.12.09.  Things Loc planned to add after the first draft:
  \\
  \ding{253} images from \cite{Phuong.2019},\cite{Wilson.2018}, and from \cite{Loshchilov.2019}.
  \\
  \ding{253} screenshot from \cite{Reddi.2019} about their convergence of AMSGrad, ask permission, pointed out \cite{Phuong.2019}
  \\
  \ding{253} Appendix on backprop algo to compare to Goodfellow 2016
  \\ 
  \ding{253} Figure on exponential smoothing of Arabian oil (screenshot from 2019.12.03), plus two references (open text by Hyndman and a handbook related exponential smoothing)
  \\
  \ding{253} screenshots on waves of AI from Web of Science. 
  
  
	\item
	2019.12.10
	Mark: 01-motivation.tex, illustration of randomly distorted elements
	
	See Fig.\ref{fig:training-set-hexa}


  \item
	2019.12.09
	Mark: 08-recurrent.tex, LSTM cell inspired by Goodfellow


  \item
	2019.12.09
	Mark: 08-recurrent.tex, old LSTM cell
\begin{figure}[H]
	\centering
	\includegraphics[width=0.5\textwidth]{./figures/lstm_cell}
	\caption{
	Schematic representation of an LSTM cell $[n]$: In the lower part, the four gates of an LSTM cell (from left to right: \emph{forget}, \emph{input}, \emph{cell} and \emph{output gate}) are illustrated.
	Each gate consists of a fully-connected linear layer, which combines the previous hidden state $\hvt{n-1}$ and the current input $\xvt{n}$, whose output is fed into a non-linear activation function.
	On the top, the direct path that describes the evolution of the previous cell state $\cvt{n-1}$ into the new cell state $\cvt{n}$, which is governed by the output of the gates, is shown.
	{\color{red}
		[NOTE 2019.08.10.  it is best to use color to show different paths.  for example, red for the cell path, blue for the gate paths. ENDNOTE]
	}
	By multiplying component-wise the cell state $\cvt{n-1}$ with the \emph{forget-gate} output $\fvt{n}$, which has values between 0 and 1 due to the logistic sigmoid in Eq.(\ref{eq:forget-gate}), information deemed not relevant from the input $\xvt{n}$ and the hidden state $\hvt{n-1}$ would be ``forgotten'', and only relevant information would be carried forward to the new cell state $\cvt{n}$.
	\sout{By the component-wise multiplication of the output of the \emph{forget gate}, which is bounded between 0 and 1, determines to which extent the previous cell stated is carried over into the new cell state.}
	The update of the cell state is determined in two steps: By a components-wise multiplication, the output of the \emph{input gate} controls to which extent the components of the \emph{cell gate}'s output are subsequently incorporated into the new cell state. 
	To generate a new hidden state $\hvt{n}$, the new cell state $\cvt{n}$ is first normalized to the range $[-1,1]$ by a hyperbolic tangent, before it is weighted with the output of the \emph{output gate} by another component-wise multiplication.
	{\color{red} [NOTE: 2019.07.20. we need to give equation number in figure caption, such as the one added above, so to quickly identify which equation the figure corresponds to.]}
	}
	\label{fig:Olah-lstm_cell}
\end{figure}

{\color{red}
	[NOTE 2019.08.16.  we need to explain ``short-term''. 
	
	2019.08.10.  	
	we need to explain the meaning of ``forget'', ``input'', ``cell'', and ``output'' gates.
	\\   
	what does ``forget'' mean ? DONE in caption of Fig.\ref{fig:Olah-lstm_cell}.
	\\
	what does ``gate'' mean ?  a gate is a sigmoid activation function that ``squashes'' inputs onto its range.  the logistic sigmoid and the hyperbolic tangent are sigmoid functions that squash inputs into the range $(0,1)$ and $(-1, 1)$, respectively.
	\\
	what does ``input gate'' mean ?
	\\
	what does ``cell gate'' mean ?
	\\
	what does ``output gate'' mean ?
	\\
	why do we need all these gates ?
	\\
	we need answers to these questions.  it is not intuitive without explanation.  
	ENDNOTE]
}
  
  \item
2019.12.09:
Mark: 08-recurrent.tex, graph dynamical systems
Even more so if we adopt the graph representation of RNNs (Figs.\ref{fig:our-RNN} and~\ref{fig:our-RNN-2}) for the time-discrete equations of motion illustrated in Fig.\ref{fig:eom_graph}.
%
\begin{figure}[H]
	\centering
	\includegraphics[width=0.7\textwidth]{./figures/LTI_graph}
	\caption{
	{\color{blue}TODO}
	{\color{red} [NOTE: 2019.07.20. we need to give equation number in figure caption, such as the one added above, so to quickly identify which equation the figure corresponds to.]}
	}
	\label{fig:eom_graph}
\end{figure} 
  
  \item
2019.12.08
Mark: 08-recurrent.tex, additional aspects
{\color{blue} Possibly also mention the following aspects:
\begin{itemize}
\item Weights of recurrent mapping and weights of input mapping are some of most difficult parameters to learn (Goodfellow)
\item Echo state networks: learn only output weights
\item Initialization: spectral radius of Jacobian; contractivity 
\end{itemize}
}

  \item
2019.12.08
Mark: 08-recurrent.tex: RNN classification, loss function

\noindent
In classification tasks, a $\softmax$ function is typically used to compute the probabilities over the output at each time step.
\begin{equation}
\yvthat{t} = \softmax \ovt{n} ,
\label{eq:softmax-on}
\end{equation}
which is input to the loss function along with the target values $\yvt{n}$.
%
The total loss for an input sequence $\xv$ and a target sequence $\yv$ is the sum of the losses over all time steps,
%
\begin{equation}
L = \sum_t L^{(t)} .
\end{equation}
%
{\color{blue}
{\bf TODO:} back-propagation through time, gradient computation
}

  
  \item
  2019.12.08
  Mark: 08-reccurent.tex, Comment on notation and Goodfellow
  
  {\color{blue}
[NOTE: 2019.01.14.: we need to think about the notation for sequences
ENDNOTE]
}

{\color{blue}
[NOTE: 2019.01.14.: why aren't $\thetav$ and $\hvt{0}$ arguments in $g$ in Goodfellow?
ENDNOTE]
}

{\color{blue}
[NOTE: 2019.08.13: is the relation $f_2 (\bx^{[n]}) = a_2 (\bz_2^{[n]})$ really clear? what about Eq.103, do we want to keep it?
}


  \item
  2019.12.08
  Mark: 08-recurrent.tex, Comment on RNN figure
  
  \noindent
{\color{red} 
	[NOTE: 2019.08.16. HELLO Fig.\ref{fig:Goodfellow-RNN} is to be replaced by Fig.\ref{fig:our-RNN}, which is closer to the figure by \cite{Olah.2015} in his web article \href{https://colah.github.io/posts/2015-08-Understanding-LSTMs/}{Understanding LSTM Networks} (\href{https://web.archive.org/web/20190731122811/https://colah.github.io/posts/2015-08-Understanding-LSTMs/}{Internet archive}), which was referred to in the PyTorch's tutorial webpage \href{https://pytorch.org/tutorials/intermediate/char_rnn_classification_tutorial.html#classifying-names-with-a-character-level-rnn}{CLASSIFYING NAMES WITH A CHARACTER-LEVEL RNN} (\href{https://web.archive.org/web/20190510131439/https://pytorch.org/tutorials/intermediate/char_rnn_classification_tutorial.html}{Internet archive}).
	\cite{Olah.2015} called $\bh$ the ``output'' of the processor $A$, which is correct, just like the state $\by^{[n]}$ is the output of the processor $f(\cdot)$. 
	the advantage of Fig.\ref{fig:our-RNN} over the equivalent figure in Colah's \href{https://colah.github.io/posts/2015-08-Understanding-LSTMs/}{Understanding LSTM Networks} (\href{https://web.archive.org/web/20190731122811/https://colah.github.io/posts/2015-08-Understanding-LSTMs/}{Internet archive}) is that the number of delay steps is explicitly represented.
	ENDNOTE]
}.

  
  \item   
  2020.04.15.  move the section on cybernetics and the 3 waves of AI back into the text as an Appendix.
  
  2019.12.07
  Mark: 20-history.tex, subsection up and down of AI, cybernetics, etc., moved to NOTES
  

  
  \item
  2019.12.04
  Mark: 08-recurrent.tex, note on higher order derivatives
  
  {\color{red}
	[NOTE: 2019.01.23. updated 2019.02.03.
	this note could be added as a remark after we introduce the concept of increasing
	the size of the matrix $\mathbf{ h }$ to decrease the test (generalization) error.
	the use of  
	higher-order derivatives to develop time-integration schemes is akin to increasing the size of the matrix $\mathbf{ h }$ in RNNs.
	for example,
	\cite{Mohazzabi.2017} use Taylor series with higher-order derivatives to develop a time-integration scheme for general first-order ODEs
	\begin{align}
		\frac { \mathrm { d } y } { \mathrm { d } x } = f ( x , y )
		\label{eq:ODE}
	\end{align}
	the Taylor series about the point $x_n$, with $h$ being the increment such that $x_{n+1} = x_n + h$, is given by
	\begin{align}
		y _ { n + 1 } = y _ { n } + \frac { y _ { n } ^ { ( 1 ) } } { 1 ! } h + \frac { y _ { n } ^ { ( 2 ) } } { 2 ! } h ^ { 2 } + \frac { y _ { n } ^ { ( 3 ) } } { 3 ! } h ^ { 3 } + \frac { y _ { n } ^ { ( 4 ) } } { 4 ! } h ^ { 4 } + \cdots
	\end{align}
	subsequent differentiations of (\ref{eq:ODE}) yield
	\begin{align}
		y ^ { ( 1 ) } & = f ( x , y )
		\\
		y ^ { ( 2 ) } & = \frac { \partial f } { \partial x } + \frac { \partial f } { \partial y } y ^ { ( 1 ) }
		\\
		y ^ { ( 3 ) } & = \frac { \partial ^ { 2 } f } { \partial x ^ { 2 } } + 2 \frac { \partial ^ { 2 } f } { \partial x \partial y } y ^ { ( 1 ) } + \frac { \partial ^ { 2 } f } { \partial y ^ { 2 } } \left( y ^ { ( 1 ) } \right) ^ { 2 } + \frac { \partial f } { \partial y } y ^ { ( 2 ) }	
		\\
		y ^ { ( 4 ) } & = \frac { \partial ^ { 3 } f } { \partial x ^ { 3 } } + 3 \left( \frac { \partial ^ { 3 } f } { \partial x ^ { 2 } \partial y } + \frac { \partial ^ { 3 } f } { \partial x \partial y ^ { 2 } } y ^ { ( 1 ) } \right) y ^ { ( 1 ) } + \frac { \partial ^ { 3 } f } { \partial y ^ { 3 } } \left( y ^ { ( 1 ) } \right) ^ { 3 }
		\nonumber
		\\
		& + 3 \left( \frac { \partial ^ { 2 } f } { \partial x \partial y } + \frac { \partial ^ { 2 } f } { \partial y ^ { 2 } } y ^ { ( 1 ) } \right) y ^ { ( 2 ) } + \frac { \partial f } { \partial y } y ^ { ( 3 ) }
		\\
		\text{etc.}
		\nonumber
	\end{align}
	
	in structural dynamics,
	\cite{Hoff1990a} employed higher-order derivatives to derive one-step time-integration algorithms with higher-order accuracies.
	when restricted to third-order derivatives for the simplicity of presenting the main idea, they approximated the displacements at time $t$ in the time interval $[t_n , \, t_{n+1}]$, with $\tau := t - t_n$ and $\Delta t := t_{n+1} - t_n$ as follows
	as follows	
	\begin{align}
		\mathbf { d } ( \tau ) & = \mathbf { d } _ { \mathrm { n } } + \mathbf { d } _ { n } \tau + \beta _ { 2 } \mathbf { \ddot { d } } _ { n } \tau ^ { 2 } + \beta _ { 3 } \frac { \Delta \mathbf { \ddot { d } } } { \Delta t } \tau ^ { 3 }
		\label{eq:Hoff-displacements-1}
		\\
		\mathbf { \dot d } ( \tau ) & = \mathbf { \dot { d } } _ { n } + \mathbf { \ddot { d } } _ { n } \tau + \gamma _ { 2 } \frac { \Delta \mathbf { \ddot { d } } } { \Delta t } \tau ^ { 2 }
		\\
		\mathbf { \ddot { d } } ( \tau ) & = \mathbf { \ddot { d } } _ { n } + \frac { \Delta \mathbf { \ddot { d } } } { \Delta t } \tau
		\label{eq:Hoff-displacements-3}
	\end{align}	
	in the same manner, they approximated the velocities as follows
	\begin{align}
		\mathbf { v } ( \tau ) & = \mathbf { v } _ { n } + \mathbf { \dot { v } } _ { n } \tau + \eta _ { 2 } \mathbf { \ddot { v } } _ { n } \tau ^ { 2 } + \eta _ { 3 } \frac { \Delta \mathbf { \ddot { v } } } { \Delta t } \tau ^ { 3 }
		\label{eq:Hoff-velocities-1}
		\\
		\mathbf{ \dot { v } } ( \tau ) & = \mathbf{ \dot { v } } _ { n } + \mathbf { \ddot { v } } _ { n } \tau + \kappa _ { 2 } \frac { \Delta \mathbf { \ddot { v } } } { \Delta t } \tau ^ { 2 }
		\\
		\mathbf { \ddot { v } } ( \tau ) & = \mathbf { \ddot { v } } _ { n } + \frac { \Delta \mathbf { \ddot { v } } } { \Delta t } \tau
		\label{eq:Hoff-velocities-3}
	\end{align}
	the above six ``state vectors'' were then substituted in the equations of motion in first-order form (\ref{eq:EoM-1st-order-form-a}) or (\ref{eq:EoM-1st-order-form-b}) to obtain two equations to solve for the two increments $\Delta \mathbf { \ddot { d } }$ and $\Delta \mathbf { \ddot { v } }$.
	moreover, the following ``reasonable equations'' were assumed for use in the six approximations (\ref{eq:Hoff-displacements-1})-(\ref{eq:Hoff-velocities-3}) and in the two equations for $\Delta \mathbf { \ddot { d } }$ and $\Delta \mathbf { \ddot { v } }$:
	\begin{align}
		\mathbf { \dot d } _ { n } & = \mathbf { v } _ { n }
		\\
		\mathbf { \ddot d } _ { n } & = \mathbf { \dot v } _ { \mathrm { n } }
		\\
		\mathbf { \dot v } _ { \mathbf { n } } & = \mathbf { M } ^ { - 1 } \left[ \mathbf { p } _ { \mathbf { n } } - \mathbf { C } \mathbf { v } _ { \mathbf { n } } - \mathbf { K } \mathbf { d } _ { n } \right]
	\end{align}

	\noindent
	ENDNOTE]

}

  
  \item 
  2019.12.03.
  Mark: 01-motivation.tex, questions to Oishi, Barlow points, reduced integration
  
  {\color{red}
  	[NOTE: 2018.10.29.  we need to email to Oishi today with a request to use their figures, and at most two questions to start the communication.  don't wait till we have a long list of questions, since that would take him more time to reply.  we need their permission to use their figures ASAP.
  	ENDNOTE]
  }
  
  \vspace{12pt}
  {\color{red}
  	[NOTE: 2018.10.18.  we need to discuss: 
  	
  	(1) Barlow points and accuracy in strain computation (this could be an advantage of having more accurate integration equivalent to full integration while using only reduced-integration points), 
  	
  	(2) reduced integration without stabilization should never be used in industry setting due to its instability; that's why there was a movenent to develop elements without shear / volume locking  with full integration, thus avoiding instability; refer to Vu-Quoc et al.
  	%\cite{Vu-Quoc.1989:rd1948}, \cite{Vu-Quoc.1990:rd2555}, \cite{Vu-Quoc.1992:rd7232} on spurious mode stabilization, and to \cite{Vu-Quoc.2003:rd1634}, \cite{Vu-Quoc.2003:rd1509}, \cite{Vu-Quoc.2013:rd4592} on solid shells.
  	
  	(3) we need to include the table in \cite{Oishi.2017:rd9648} showing training error and test error to connect to \cite{Goodfellow.2016}, pdf p.135, Fig.5.3 on ``Typical relationship between capacity and error'': see, e.g., Table 1 in \cite{Oishi.2017:rd9648}; please retype this table, which also gave the architecture of their network (depth and width).
  	
  	(4) we need to include the parameterization of element distortion in \cite{Oishi.2017:rd9648} to explain how they generated their dataset to train their network: See, e.g., Fig.7 in \cite{Oishi.2017:rd9648}.
  	
  	(5) please study Table 2 in \cite{Oishi.2017:rd9648}; there are some nice results there.
  	
  	ENDNOTE]
  }
  
  \vspace{12pt}
  {\color{red}
  	[NOTE: 2018.10.18.  Questions to Oishi:
  	
  	\begin{itemize}
  		
  		\item \sout{which activation function were used in their network ?  ReLU or sigmoid ?}
  		
  		\item in Table 1 in \cite{Oishi.2017:rd9648}, what is the error using the regular Gauss-Legendre weights, with the same number of integration points ?
  		
  		\item please send us any finite-element examples that used this new method, compared to the old method of integration, to give a feel for the improvement.
  		
  	\end{itemize}
  	
  	ENDNOTE]
  }
  
  \vspace{12pt}
  {\color{red} 
  	[NOTE: 2018.10.17.  we should leave in this Motivation section only  new / novel, very short and concise, applications of DL, and move all reviews to Section~\ref{sc:history} on Historical perspective.  
  	ENDNOTE]
  }
  
    
  \item 2019.07.26.  ``sigmoid function'' is a general class of functions, which includes the logistic sigmoid, hyperbolic tangent, and more; see Wikipedia, `Sigmoid function', \href{https://en.wikipedia.org/w/index.php?title=Sigmoid_function&oldid=904189722}{version 15:22, 30 June 2019}.   we should always have the adjective ``logistic'' when we refer to the logistic sigmoid function, and not just ``sigmoid function'' to avoid confusion, since the hyperbolic tangent is also a sigmoid function.
  see also \cite{Goodfellow.2016}, p.xxii (pdf p.23), p.65 (pdf p.88), p.169 (pdf p.212).
   
  \item 2019.04.06. i was reading about the principle of maximum likelihood to understand the maximum likelihood cost function in Eq.(\ref{eq:likelihood-cost}) in \cite{Goodfellow.2016}, pdf p.196.
  \cite{Goodfellow.2016}, Section 5.5.1, pdf p.152, about ``Conditional log-likelihood and mean squared error'' and ``linear regression as maximum likelihood'', wrote: ``if $\boldsymbol{X}$ represents all of our inputs and $\boldsymbol{Y}$ all our observed \underline{{\em targets}}, then the conditional maximum likelihood estimator is''
  \begin{align}
  	\bparams{ML}
  	=
  	\arg\max_{\boldsymbol{\theta}} 
  	P( \boldsymbol{X} \mid \boldsymbol{Y} ; \bparam)
  \end{align} 
  and ``if the examples are assumed to be independent and identically distributed, then $\boldsymbol{\theta}_{ML}$ can be decomposed into''
  \begin{align}
  	\boldsymbol{\theta}_{ML}
  	=
  	\arg\max_{\boldsymbol{\theta}}
  	\sum_{i=1}^m \log p (\byp{i} \mid \bxp{i} ; \bparam)
  \end{align}
  further \cite{Goodfellow.2016}, pdf p.153, wrote that linear regression is ``an algorithm that learns to take the input $\bx$ and produce an output value $\hat{\y}$''.
  then i realized the difference between our current notation for outputs and that used in \cite{Goodfellow.2016}, and made some adjustments to avoid confusion as listed below: 
  \begin{enumerate}
  	
  	\item
  	for the network {\em predicted} or {\em approximated} output, 
  	\cite{Goodfellow.2016} used $\hat{y}$, whereas we will use $\widetilde{y}$ for scalar and $\widetilde{\by}$ for matrix, with the tilde used to indicate an approximation, similar to the symbol $\approx$.
  	
  	\item
  	for the target output, 
  	\cite{Goodfellow.2016} used $y$ for scalar and matrix $\by$ for matrix.  
  	note that $\by$ is part of the data ($\bx , \by$) to train or to validate the network.
  	we will use the same notation.  (initially, i used $\byp{L} = \by$ as output of the last layer $L$, but realized that this notation could be confusing.  so instead, we will use $\byp{L} = \widetilde{\by}$ or $\byp{L} = \bout$ (with the tilde closer to $\by$) as network predicted output.  i need to go back to the figures to change the notation to this last one.)
  	
  	\item 
  	for the
  	expanded predicted output matrix, we will use 
  	% $\expOut{\nwidetilde{\by}}$,
  	$\expOut{\bout}$,  
  	% $\overline{\widetilde{\by}}$, 
  	or
  	$\expand{\bout}$.
  	i suggest we use $\expand{\bout}$ to leave space above the whole character in case we need overhead dots (e.g., $\nddt{\expand{\bout}}$) or something like that.\footnote{the new notation using the {\em em} font size unit also scales well with the text fontsize in footnotes, e.g., $\expand{\bout}$, $\nddt{\expand{\bout}}$}
  	
  \end{enumerate} 
  
  \item 2018.12.12 : the references to Furshpan's articles seem to be broken for some reason. The document does not compile any more. I put those references in a separate bib file to save them.
    
  \item 2018.11.06 : we need to give the page number when we refer to a book for a specific information to save for time for us and for the readers when such info needs to be looked up in the book; see footnote~\ref{fn:pageNumber}. 
  
  \item 2018.11.01 : consolidated bib files to reduce the number of files to less than 60, which is the limit for a free Overleaf account.
  
  \item 2018.10.30 : introduced package \verb+enumitem+ to customize enumerations.   
  Using the optional flag \verb+resume+, the numbering of lists can be resumed
  \begin{enumerate}
    \item first
    \item second
  \end{enumerate}
  from previous lists:
  \begin{enumerate}[resume]
    \item third
  \end{enumerate}
  With the flag \verb+start=42+, we can set the number of the first item in an enumeration:
  \begin{enumerate}[start=42]
  \item forty-second 
  \end{enumerate}
  
  \item 2018.10.15 : introduced package \verb+caption+ to reduce the width of the figure / table captions.
  
  \item 2018.10.15 : introduced package \verb+siunitx+ for numbers with/without units.
  
  \item 2018.10.14: two-href problem solved; the problem was that i skipped one level of section by mistake, i.e., i went from ``section'' to ``subsubsection'', without having a ``subsection'' in between.  2018.10.11.  i had to use two href commands side by side for href to work.  what was the problem ?
  
  \item 2018.10.08: added tikz plots for activation functions: rectified linear unit and derivatives, logistic sigmoid, hyperbolic tangent.  
  
  \item 2018.08.26: included package \verb+yyyymmdd+ for ISO date format ``yyyy.mm.dd''
  
  \item 2018.08.26: included package \verb+ulem+ for strikeout font \sout{Hello} \sout{{\em Hello}} \sout{{$\alpha \beta \gamma$}} using the command \verb+\sout+ for in-line equation. on the other hand, for stand-alone equations, use the command \verb+\xout+ to get \xout{{$\alpha \beta \gamma$}}, since the command \verb+\sout+ just underlines the equations.  it is better, however, to use the command \verb+\cancel+ in the package \verb+cancel+ to get $\cancel{\alpha \beta \gamma}$, which is a clearer cancelation or deletion.  see Eq.(\ref{eq:cancel}) for an example.

  {\color{red}
  \begin{align}
      \label{eq:cancel}
      \boxit{
        \sout{
        v = 0 \textrm{ on } \partial \Omega
        }
        \quad
        \xout{
        v = 0 \textrm{ on } \partial \Omega
        }
        \quad
        \cancel{
        v = 0 \textrm{ on } \partial \Omega
        }
      }
      \quad
      \text{ NOT CORRECT! }
  \end{align}
  } 
    
  % \item include package \verb+dingbat+ for the pointing finger icon $\leftpointright$ using \verb+$\leftpointright$+
  
\end{itemize}

}

\begin{rem}
	here is an example of using the Remark environment ``rem'' defined in main.tex.
	by default, the remark is in italics, due to the use of the \verb+\newtheorem+ command.  
	to have Roman font, use the command \verb+\rm+, as in the
	\rm
	following example.  
	end the remark with a right-justified square ``$\square$'' using the command
	\verb+\hfill$\blacksquare$+.
	\hfill$\blacksquare$ 
\end{rem}


==> 16-other-apps.tex <==

\section{Other applications of deep learning}
\label{sc:other-apps}

\subsection{Inverse problem in material design}

\cite{Sanchez.2018:rd0001} is a Science paper.

\subsection{Structural health monitoring}

\cite{Wu.1992:rd0001} is an early adoption of neural networks for structural health monitoring.

\cite{Khan.2018:rd0001} recent review of deep learning applied to structural health management.


\subsection{Model selection and error estimation}

\cite{Oneto.2018:rd1035}
\href{https://drive.google.com/open?id=1gJbIWtY-SELREoP2zmVeDm-7Nh1hPfit}{(pdf)}


\section{Other data-driven approaches}

\subsection{Distance minimization, variational approach}

\cite{Nguyen.2018:rd1573}
(\href{https://drive.google.com/open?id=1iHzrjw2Iv_TX103ydpNEFqAUVvoqu7v2}{pdf})

\subsection{NOT yet classified}

\cite{Wang.2018:rd9683}

\cite{Paulson.2018:rd1011}

\cite{Du.2018:rd1167}



==> macros_alex.tex <==
\newcommand{\alex}[1]{{\color{blue}#1}}
%\newcommand{\dx}{\mathrm dx}
\newcommand{\dxi}{\mathrm d \xi}
\newcommand{\deta}{\mathrm d \eta}
\newcommand{\dzeta}{\mathrm d \zeta}

\newcommand{\dx}{\mathrm dx}
\newcommand{\dy}{\mathrm dy}
\newcommand{\dz}{\mathrm dz}

%\newcommand{\xvf}{\boldsymbol x^{(1)}}


\newcommand{\gt}{g^{(t)}}

\newcommand{\av}{\boldsymbol a}
\newcommand{\avt}[1]{\boldsymbol a^{(#1)}}
%\newcommand{\bv}{\boldsymbol b}
\newcommand{\bv}{\boldsymbol b}
\newcommand{\cv}{\boldsymbol c}
\newcommand{\dv}{\boldsymbol d}
\newcommand{\fv}{\boldsymbol f}
%<<<<<<< Updated upstream
\newcommand{\gv}{\boldsymbol g}
\newcommand{\gvt}[1]{\gv^{(#1)}}
\newcommand{\hv}{\boldsymbol h}
\newcommand{\hvt}[1]{\hv^{(#1)}}
\newcommand{\iv}{\boldsymbol i}
\newcommand{\ivt}[1]{\iv^{(#1)}}
%=======
%\newcommand{\hv}{\boldsymbol h}
%\newcommand{\hvt}[1]{\boldsymbol h^{(#1)}}
%>>>>>>> Stashed changes
\newcommand{\jv}{\boldsymbol j}
\newcommand{\ovt}[1]{\boldsymbol o^{(#1)}}
\newcommand{\uv}{\boldsymbol u}
\newcommand{\vv}{\boldsymbol v}
\newcommand{\xv}{\boldsymbol x}
\newcommand{\xvt}[1]{\boldsymbol x^{(#1)}}
\newcommand{\yv}{\boldsymbol y}
\newcommand{\yvthat}[1]{\hat{\yv}^{(#1)}}
\newcommand{\yvt}[1]{\boldsymbol y^{(#1)}}
\newcommand{\zv}{\boldsymbol z}

\newcommand{\thetav}{\boldsymbol \theta}

\newcommand{\Wm}{\boldsymbol W}
\newcommand{\Um}{\boldsymbol U}
\newcommand{\Vm}{\boldsymbol V}

\newcommand{\Am}{\boldsymbol A}
\newcommand{\Bm}{\boldsymbol B}
\newcommand{\Cm}{\boldsymbol C}
\newcommand{\Dm}{\boldsymbol D}

\DeclareMathOperator{\softmax}{softmax}

\newcommand{\Mm}{\boldsymbol M}
\newcommand{\I}{\boldsymbol I}
%\newcommand{\Dm}{\boldsymbol D}
%\newcommand{\Cm}{\boldsymbol C}
%<<<<<<< Updated upstream
\newcommand{\deltat}{\Delta t}

\newcommand{\sigmoid}{\sigma}
\newcommand{\fvt}[1]{\fv^{(#1)}}
\newcommand{\cvt}[1]{\cv^{(#1)}}
\newcommand{\bvf}{\bv_f}
\newcommand{\bvi}{\bv_i}
\newcommand{\bvg}{\bv_g}
\newcommand{\bvo}{\bv_o}
\newcommand{\Wmf}{\Wm_f}
\newcommand{\Wmi}{\Wm_i}
\newcommand{\Wmg}{\Wm_g}
\newcommand{\Wmo}{\Wm_o}
\newcommand{\Umf}{\Um_f}
\newcommand{\Umi}{\Um_i}
\newcommand{\Umg}{\Um_g}
\newcommand{\Umo}{\Um_o}
%=======
%\newcommand{\deltat}{\Delta t}
%>>>>>>> Stashed changes

